Covered Clause Elimination

Generalizing the novel clause elimination procedures developed in [M. Heule, M. J\"arvisalo, and A. Biere. Clause elimination procedures for CNF formulas. In Proc. LPAR-17, volume 6397 of LNCS, pages 357-371. Springer, 2010.], we introduce explicit (CCE), hidden (HCCE), and asymmetric (ACCE) variants of a procedure that eliminates covered clauses from CNF formulas. We show that these procedures are more effective in reducing CNF formulas than the respective variants of blocked clause elimination, and may hence be interesting as new preprocessing/simplification techniques for SAT solving.

==> defs.tex <==
\newcommand{\todo}[1]{{$\langle\!\langle$\marginpar{$\blacksquare$}\textsf{#1}$\rangle\!\rangle$}}
\newcommand{\tuple}[1]{{\langle{#1}\rangle}}
\newcommand{\setdef}[2]{{\left\{#1\,\mid \,#2\right\}}}

\newcommand{\toolname}[1]{\textsc{#1}}
\newcommand{\bclimmat}{\toolname{BCLimmat}}
\newcommand{\bczchaff}{\toolname{BCzChaff}}
\newcommand{\bcminisat}{\toolname{BCMiniSAT}}
\newcommand{\limmat}{\toolname{Limmat}}
\newcommand{\zchaff}{\toolname{zChaff}}
\newcommand{\minisat}{\toolname{MiniSAT}}
\newcommand{\bccnf}{\toolname{bc2cnf}}
\newcommand{\bcedimacs}{\toolname{bc2edimacs}}
\newcommand{\edimacsbc}{\toolname{edimacs2bc}}
\newcommand{\desbc}{\toolname{des2bc}}
\newcommand{\genfacbm}{\toolname{genfacbm}}


%\newcommand{\qed}{\hfill $\Box$}
\newcommand{\compl}{\bar}
\newcommand{\fanout}{\mathsf{fanout}}
\newcommand{\flow}{\mathsf{flow}}
\newcommand{\degree}{\mathsf{degree}}
\newcommand{\children}{\mathsf{children}}
\newcommand{\parents}{\mathsf{parents}}
\newcommand{\vars}{\mathsf{vars}}
\newcommand{\clauset}{F}
\newcommand{\circt}{\mathsf{circuit}}
\newcommand{\cnf}{\mathsf{cnf}}
\newcommand{\PHP}{{\rm PHP}_n^{n+1}}
\newcommand{\EPHP}{{\rm EPHP}_n^{n+1}}
\newcommand{\EXT}{{\rm EXT}}
\newcommand{\E}{{\rm E}}
\newcommand{\XORUNSAT}{{\rm XOR\mbox{-}UNSAT}_n}
\newcommand{\XOR}{{\rm XOR}_n}
\newcommand{\UNSAT}{{\rm UNSAT}}
\newcommand{\dom}{\textsf{domain}}
\newcommand{\up}{\textsc{up}}
\newcommand{\CL}{\mathsf{CL}}
\newcommand{\TRES}{\mathsf{T\mbox{\sf -}RES}}
\newcommand{\RES}{\mathsf{RES}}
\newcommand{\CLm}{\mathsf{CL\mbox{-}\;\!\mbox{-}}}
\newcommand{\DPLL}{\mathsf{DPLL}}
\newcommand{\inputs}{\mathsf{inputs}}
\newcommand{\outputs}{\mathsf{outputs}}
\newcommand{\shared}{\textsf{\small shared}}
\newcommand{\gate}{g}
\newcommand{\gatei}[1]{g_{#1}}
\newcommand{\fname}[1]{\textsc{#1}}
\newcommand{\FALSE}{\fname{false}}
\newcommand{\TRUE}{\fname{true}}
\newcommand{\NOT}{\fname{not}}
\newcommand{\DEF}{\fname{def}}
\newcommand{\IMPLY}{\fname{imply}}
\newcommand{\AND}{\fname{and}}
\newcommand{\OR}{\fname{or}}
\newcommand{\EVEN}{\fname{even}}
\newcommand{\ODD}{\fname{xor}}
\newcommand{\EQUIV}{\fname{equiv}}
\newcommand{\ITE}{\fname{ite}}
\newcommand{\CARD}[2]{\fname{card}_{#1}^{#2}}
%\newcommand{\CARD}[2]{\fname{card[#1,#2]}}
\newcommand{\mdef}{\mathrel{:=}}
\newcommand{\Gates}{G}
\newcommand{\CCircuit}{\mathcal{C}^\ta}
\newcommand{\Circuit}{\mathcal{C}}
\newcommand{\edges}[1]{E(#1)}
\newcommand{\graph}[1]{\textit{graph}(#1)}
\newcommand{\mfalse}{\textup{\textbf{f}}}
\newcommand{\mtrue}{\textup{\textbf{t}}}
%\newcommand{\mfalse}{\textup{\textbf{false}}}
%\newcommand{\mtrue}{\textup{\textbf{true}}}
%\newcommand{\mfalse}{\bot}
%\newcommand{\mtrue}{\top}
\newcommand{\ta}{\tau}
\newcommand{\polf}[2]{\mathsf{pol}_{#1}^{#2}}
\newcommand{\pol}{\mathsf{pol}_{\Circuit}^{\ta}}
\newcommand{\cnfgate}{{\mathbf g}}
\newcommand{\cnfgatei}[1]{{\mathbf g}_{#1}}


\newcommand{\resolve}{\otimes}

\newcommand{\rc}{\mathrm{RC}}
\newcommand{\ri}{\mathrm{RI}}

\newcommand{\binbla}{\mathrm{BLA}_2}
\newcommand{\binbca}{\mathrm{BCA}_2}

\newcommand{\ihte}{e\mathrm{HTE}}

\newcommand{\impg}{\mathsf{BIG}}
\newcommand{\lits}{\mathsf{lits}}
\newcommand{\elr}{\mathrm{ELS}}


\newcommand{\lit}{\mathrm{LIT}}
\newcommand{\sce}{\mathrm{SCE}}
\newcommand{\abce}{\mathrm{ABCE}}
\newcommand{\hcce}{\mathrm{HCCE}}
\newcommand{\acce}{\mathrm{ACCE}}
\newcommand{\hbce}{\mathrm{HBCE}}
\newcommand{\ace}{\mathrm{ATE}}
\newcommand{\te}{\mathrm{TE}}
\newcommand{\ase}{\mathrm{ASE}}
\newcommand{\se}{\mathrm{SE}}
\newcommand{\sse}{\mathrm{SSE}}
\newcommand{\hla}{\mathrm{HLA}}
\newcommand{\ala}{\mathrm{ALA}}
\newcommand{\ssa}{\mathrm{HLA}}
\newcommand{\hte}{\mathrm{HTE}}
\newcommand{\hse}{\mathrm{HSE}}
\newcommand{\flc}{\mathrm{FLC}}
\newcommand{\fle}{\mathrm{FLE}}
\newcommand{\bcp}{\mathrm{BCP}}
\newcommand{\gte}{\mathrm{GTE}}
\newcommand{\fre}{\mathrm{FRE}}
\newcommand{\cle}{\mathrm{CLE}}
\newcommand{\cla}{\mathrm{CLA}}
\newcommand{\cce}{\mathrm{CCE}}

\newcommand{\cupdot}{\mathrel{\mathop{\cup}\limits^{.}}}

\newcommand{\pl}{\mathrm{PL}}
\newcommand{\pg}{\mathrm{PG}}
\newcommand{\bce}{\mathrm{BCE}}
\newcommand{\ve}{\mathrm{VE}}
\newcommand{\coi}{\mathrm{COI}}
\newcommand{\nsi}{\mathrm{NSI}}
\newcommand{\mir}{\mathrm{MIR}}
\newcommand{\tseitin}{\mathrm{TST}}

%\newtheorem{theorem}{Theorem}[chapter]
%\newtheorem{lemma}{Lemma}[chapter]
%\newtheorem{corollary}{Corollary}[chapter]
%\newtheorem{definition}{\bf Definition}[chapter]
%\newtheorem{example}{\bf Example}[chapter]
%\newtheorem{proposition}{\bf Proposition}
\newtheorem{fact}{\bf Fact}
%\newtheorem{remark}{Remark}
%\newenvironment{proof}[0]{\textbf{Proof.} }

%-------------------- environment definitions -----------------
%\newenvironment{proposition}[0]{\begin{Proposition}}{\end{Proposition}}
%\newenvironment{example}[0]{\begin{Example} \it}{\end{Example}}
%\newenvironment{proof}[1]{\noindent{\bf Proof of #1. }}{\hfill $\Box$}
%\newenvironment{definition}{\begin{Definition} }
%{\end{Definition}}

